MAC-VO: Metrics-aware Covariance for Learning-based Stereo Visual Odometry

We propose the MAC-VO, a novel learning-based stereo VO that leverages the learned metrics-aware matching uncertainty for dual purposes: selecting keypoint and weighing the residual in pose graph optimization. Compared to traditional geometric methods prioritizing texture-affluent features like edges, our keypoint selector employs the learned uncertainty to filter out the low-quality features based on global inconsistency. In contrast to the learning-based algorithms that model the scale-agnostic diagonal weight matrix for covariance, we design a metrics-aware covariance model to capture the spatial error during keypoint registration and the correlations between different axes. Integrating this covariance model into pose graph optimization enhances the robustness and reliability of pose estimation, particularly in challenging environments with varying illumination, feature density, and motion patterns. On public benchmark datasets, MAC-VO outperforms existing VO algorithms and even some SLAM algorithms in challenging environments. The covariance map also provides valuable information about the reliability of the estimated poses, which can benefit decision-making for autonomous systems.

==> Sections/Table/Archive/EuRoC.tex <==
% \begin{table*}[htbp]
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{cccccccccccccc}
% \toprule
%   & \multicolumn{2}{c}{{ORB-SLAM3}} & \multicolumn{2}{c}{{iSLAM-VO}} & \multicolumn{2}{c}{{TartanVO(S)}} & \multicolumn{2}{c}{{DPVO}$^\star$} & \multicolumn{2}{c}{{DROID-SLAM(S)}$^\star$} & \multicolumn{2}{c}{\textbf{Ours}} \\
% \cmidrule{2-14}
%  Traj.  &  {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} \\
%  \midrule 
% MH01  & \underline{0.0061}    & \underline{0.0204}    & 0.0502 & 0.1186 & 0.6271 & 1.3888 & 0.0096          & 0.0320       & \textbf{0.0050} & \textbf{0.0098} & 0.0205       & 0.0420          \\
% MH02  & \underline{0.0043}    & \underline{0.0153}    & 0.0360 & 0.0956 & 0.4777 & 1.4331 & 0.0077          & 0.0264       & \textbf{0.0030} & \textbf{0.0100} & 0.0132       & 0.0325          \\
% MH03  & \textbf{0.0053} & \underline{0.0329}    & 0.0388 & 0.0991 & 0.7474 & 2.3390 & 0.0069          & 0.0360       & 0.0313          & 0.0397          & \underline{0.0057} & \textbf{0.0316} \\
% MH04  & \underline{0.0037}    & \textbf{0.0333} & 0.0274 & 0.1237 & 0.5269 & 2.2669 & 0.0055          & \underline{0.0339} & \textbf{0.0030} & 0.0401          & 0.0069       & 0.0419          \\
% MH05  & \underline{0.0034}    & \textbf{0.0266} & 0.0250 & 0.1176 & 0.4995 & 2.2997 & 0.0056          & \underline{0.0345} & \textbf{0.0028} & 0.0358          & 0.0071       & 0.0381          \\
% V101 & \underline{0.0404}    & \underline{0.0868}    & 0.0728 & 0.1321 & 1.1814 & 1.4619 & 0.0650          & 0.0951       & \textbf{0.0363} & \textbf{0.0344} & 0.0439       & 0.0916          \\
% V102 & 0.0166          & 0.0610          & 0.0535 & 0.0991 & 1.1279 & 1.5005 & 0.0192          & 0.0778       & \textbf{0.0079} & \textbf{0.0111} & \underline{0.0128} & \underline{0.0442}    \\
% V103 & 0.0482          & 0.0916          & 0.0781 & 0.1403 & 1.5064 & 1.0126 & 0.0264          & \underline{0.0441} & \textbf{0.0105} & \textbf{0.0178} & \underline{0.0216} & 0.0449          \\
% V201 & 0.0885          & 0.0664          & 0.0867 & 0.1007 & 1.1121 & 1.2497 & \underline{0.0189}    & 0.0422       & \textbf{0.0153} & \textbf{0.0161} & 0.0236       & \underline{0.0342}    \\
% V202 & 0.0293          & 0.0535          & 0.0650 & 0.1192 & 1.0840 & 1.3692 & \textbf{0.0146} & 0.0306       & \underline{0.0154}    & \textbf{0.0089} & 0.0203       & \underline{0.0258}    \\
% V203 & 0.3765          & 0.3936          & 0.1147 & 0.2121 & 1.5461 & 1.8567 & \underline{0.0188}    & \underline{0.0491} & \textbf{0.0125} & \textbf{0.0117} & 0.0334 & 0.0508 \\
% \midrule 
% Avg.    & 0.0566          & 0.0801          & 0.0589 & 0.1235 & 0.9488 & 1.6525 & \underline{0.0180}    & 0.0456       & \textbf{0.0130} & \textbf{0.0214} & 0.0190       & \underline{0.0434}   \\

% \bottomrule
% \end{tabular}
% }
% \caption{Performance comparison of different methods on the EuRoC Dataset.\\\\
%         \small{$^\star$ The estimated sequence is scale-aligned with ground truth}}
% \end{table*}


\begin{table*}[htbp]
\centering
\captionsetup{font=small}
\caption{Relative Motion Error on the EuRoC Dataset.}
\vspace{-2mm}
\resizebox{\linewidth}{!}{\begin{tabular}{lcccccccccccc}
\multicolumn{10}{l}{\textbf{Relative Translation Error ($t_{\mathrm{rel}}, \mathrm{m} / \mathrm{frame}$)}}\\
\toprule
Trajectory & MH01 & MH02 & MH03 & MH04 & MH05 & V101 & V102 & V103 & V201 & V202 & V203 & Avg.\\
\midrule
\textbf{SLAM} \\
\hspace{3mm}ORB-SLAM 3                & 0.0035   & 0.0036   & 0.0058   & 0.0061   & 0.0059   & 0.0049   & 0.0096   & 0.0137   & 0.0064   & 0.009    & 0.033    & 0.0092\\
\hspace{3mm}DROID-SLAM$^\star$        & \textbf{0.0012} & \textbf{0.0012} & 0.0034   & 0.0031   & \textbf{0.0025} & \textbf{0.0024} & \textbf{0.0026} & 0.0036   & \textbf{0.0012} & \textbf{0.0017} & \textbf{0.0034} & \textbf{0.0024}\\
\midrule
\textbf{VO} \\
\hspace{3mm}iSLAM-VO                  & 0.0042   & 0.0041   & 0.0076   & 0.0082   & 0.0070   & 0.0041   & 0.0066   & 0.0088   & 0.004    & 0.0078   & 0.0151   & 0.0071\\
\hspace{3mm}TartanVO$^{\star\dagger}$ & 0.0121   & 0.0172   & 0.0302   & 0.0213   & 0.0193   & 0.0124   & 0.0251   & 0.0263   & 0.0065   & 0.0171   & 0.0303   & 0.0198\\
\hspace{3mm}TartanVO                  & 0.0277   & 0.0289   & 0.0514   & 0.0501   & 0.0464   & 0.0224   & 0.0394   & 0.0351   & 0.0195   & 0.0361   & 0.0473   & 0.0368\\
\hspace{3mm}DPVO$^{\star\dagger}$     & 0.0015   & 0.0014   & \underline{0.0028} & \underline{0.0029} & \underline{0.0028} & \underline{0.0026} & 0.0041   & \underline{0.0033} & \underline{0.0016} & 0.0022   & \underline{0.0045} & \underline{0.0027}\\
\midrule
\textbf{Ours}                         & \underline{0.0014} & \underline{0.0013} & \textbf{0.0023} & \textbf{0.0028} & \textbf{0.0025} & \textbf{0.0024} & \underline{0.0029} & \textbf{0.0032} & \textbf{0.0012} & \underline{0.0018} & 0.0049  & \textbf{0.0024} \\
\bottomrule
% \multicolumn{10}{l}{\small{$^\star$ The estimated sequence is scale-aligned with ground truth.}}\\
% \multicolumn{10}{l}{\small{$^\dagger$ Monocular method.}}
\end{tabular}}


\vspace{3mm}

\resizebox{\linewidth}{!}{\begin{tabular}{lcccccccccccc}
\multicolumn{10}{l}{\textbf{Relative Rotation Error ($r_{\mathrm{rel}}, {}^\circ / \mathrm{frame}$)}}\\
\toprule
Trajectory & MH01 & MH02 & MH03 & MH04 & MH05 & V101 & V102 & V103 & V201 & V202 & V203 & Avg.\\
\midrule
\textbf{SLAM} \\
\hspace{3mm}ORB-SLAM 3                & 0.0450   & 0.0495   & 0.0603   & 0.0501   & 0.0526   & 0.0888   & 0.1757   & 0.2669   & 0.1615   & 0.1528   & 0.9497  & 0.1866 \\
\hspace{3mm}DROID-SLAM$^\star$        & \textbf{0.0159} & \textbf{0.0169} & 0.2656   & \textbf{0.0224} & \textbf{0.0193} & \underline{0.0314} & \textbf{0.0417} & \underline{0.0642} & \textbf{0.0289} & \textbf{0.0399} & \textbf{0.1033} & 0.0590\\
\midrule
\textbf{VO} \\
\hspace{3mm}iSLAM-VO                  & 0.0560   & 0.0620   & 0.2789   & 0.0682   & 0.0603   & 0.0756   & 0.1241   & 0.1554   & 0.0920   & 0.1252   & 0.2984  & 0.1269 \\
\hspace{3mm}TartanVO$^{\star\dagger}$ & 0.0560   & 0.0621   & 0.2791   & 0.0681   & 0.0604   & 0.0756   & 0.1244   & 0.1552   & 0.0920   & 0.1251   & 0.2986  & 0.1270 \\
\hspace{3mm}TartanVO                  & 0.5122   & 0.5037   & 0.6635   & 0.5400   & 0.4797   & 0.5322   & 1.0420   & 1.3127   & 0.4684   & 1.1607   & 1.9657  & 0.8346 \\
\hspace{3mm}DPVO$^{\star\dagger}$     & \underline{0.0207} & 0.0212   & \underline{0.0273} & \underline{0.0264} & 0.0243   & 0.0405   & 0.0496   & 0.0662   & \underline{0.0342} & 0.0493   & \underline{0.1205} & \underline{0.0437}\\
\midrule
\textbf{Ours}                         & 0.0214   & \underline{0.0199} & \textbf{0.0238} & 0.0273   & \underline{0.0216} & \textbf{0.0304} & \underline{0.0434} & \textbf{0.058} & \textbf{0.0289} & \underline{0.0406} & 0.1284  & \textbf{0.0403} \\
\bottomrule
\multicolumn{10}{l}{\small{$^\star$ The estimated sequence is scale-aligned with ground truth.}}\\
\multicolumn{10}{l}{\small{$^\dagger$ Monocular method.}}
\end{tabular}}
\label{tab: EurocResult}
\end{table*}


==> Sections/Table/Archive/EuRoC_20240604.tex <==
\begin{table*}[htbp]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{cccccccccccccc}
\toprule
  & \multicolumn{2}{c}{{ORB-SLAM3}} & \multicolumn{2}{c}{{iSLAM-VO}} & \multicolumn{2}{c}{{TartanVO(S)}} & \multicolumn{2}{c}{{DPVO}$^\star$} & \multicolumn{2}{c}{{DROID-SLAM(S)}$^\star$} & \multicolumn{2}{c}{\textbf{Ours}} \\
\cmidrule{2-14}
 Traj.  &  {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} \\
 \midrule 
MH01  & \underline{0.0061}    & \underline{0.0204}    & 0.0502 & 0.1186 & 0.6271 & 1.3888 & 0.0096          & 0.0320       & \textbf{0.0050} & \textbf{0.0098} & 0.0205       & 0.0420          \\
MH02  & \underline{0.0043}    & \underline{0.0153}    & 0.0360 & 0.0956 & 0.4777 & 1.4331 & 0.0077          & 0.0264       & \textbf{0.0030} & \textbf{0.0100} & 0.0132       & 0.0325          \\
MH03  & \textbf{0.0053} & \underline{0.0329}    & 0.0388 & 0.0991 & 0.7474 & 2.3390 & 0.0069          & 0.0360       & 0.0313          & 0.0397          & \underline{0.0057} & \textbf{0.0316} \\
MH04  & \underline{0.0037}    & \textbf{0.0333} & 0.0274 & 0.1237 & 0.5269 & 2.2669 & 0.0055          & \underline{0.0339} & \textbf{0.0030} & 0.0401          & 0.0069       & 0.0419          \\
MH05  & \underline{0.0034}    & \textbf{0.0266} & 0.0250 & 0.1176 & 0.4995 & 2.2997 & 0.0056          & \underline{0.0345} & \textbf{0.0028} & 0.0358          & 0.0071       & 0.0381          \\
V101 & \underline{0.0404}    & \underline{0.0868}    & 0.0728 & 0.1321 & 1.1814 & 1.4619 & 0.0650          & 0.0951       & \textbf{0.0363} & \textbf{0.0344} & 0.0439       & 0.0916          \\
V102 & 0.0166          & 0.0610          & 0.0535 & 0.0991 & 1.1279 & 1.5005 & 0.0192          & 0.0778       & \textbf{0.0079} & \textbf{0.0111} & \underline{0.0128} & \underline{0.0442}    \\
V103 & 0.0482          & 0.0916          & 0.0781 & 0.1403 & 1.5064 & 1.0126 & 0.0264          & \underline{0.0441} & \textbf{0.0105} & \textbf{0.0178} & \underline{0.0216} & 0.0449          \\
V201 & 0.0885          & 0.0664          & 0.0867 & 0.1007 & 1.1121 & 1.2497 & \underline{0.0189}    & 0.0422       & \textbf{0.0153} & \textbf{0.0161} & 0.0236       & \underline{0.0342}    \\
V202 & 0.0293          & 0.0535          & 0.0650 & 0.1192 & 1.0840 & 1.3692 & \textbf{0.0146} & 0.0306       & \underline{0.0154}    & \textbf{0.0089} & 0.0203       & \underline{0.0258}    \\
V203 & 0.3765          & 0.3936          & 0.1147 & 0.2121 & 1.5461 & 1.8567 & \underline{0.0188}    & \underline{0.0491} & \textbf{0.0125} & \textbf{0.0117} & 0.0334 & 0.0508 \\
\midrule 
Avg.    & 0.0566          & 0.0801          & 0.0589 & 0.1235 & 0.9488 & 1.6525 & \underline{0.0180}    & 0.0456       & \textbf{0.0130} & \textbf{0.0214} & 0.0190       & \underline{0.0434}   \\

\bottomrule
\end{tabular}
}
\caption{Performance comparison of different methods on the EuRoC Dataset.\\\\
        \small{$^\star$ The estimated sequence is scale-aligned with ground truth}}
\end{table*}


==> Sections/Table/Archive/KITTI_20240604.tex <==
% \begin{table*}[htbp]
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{cccccccccccccc}
% \toprule
%   & \multicolumn{2}{c}{{ORB-SLAM3}} & \multicolumn{2}{c}{{iSLAM-VO}} & \multicolumn{2}{c}{{TartanVO(S)}} & \multicolumn{2}{c}{{DPVO}$^\star$} & \multicolumn{2}{c}{{DROID-SLAM(S)}$^\star$} & \multicolumn{2}{c}{\textbf{Ours}} \\
% \cmidrule{2-14}
%  Traj.  &  {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} \\
% \midrule 
% 00 & \underline{0.0018} & 0.037          & 0.0038         & 0.0877         & 0.004          & 0.1138         & 0.002          & 1.2781         & \textbf{0.0017} & \underline{0.0287} & 0.0022         & \textbf{0.0284} \\
% 01 & \underline{0.0009} & \textbf{0.0419} & 0.0022         & 0.3027         & 0.0077         & 1.4809         & \textbf{0.0006} & \underline{0.0952} & 0.001          & 0.7194         & 0.0043         & 0.2836         \\
% 02 & 0.0014         & 0.0378         & 0.0032         & 0.0795         & 0.0035         & 0.1103         & \textbf{0.0011} & 0.634          & \underline{0.0012} & \underline{0.0277} & 0.002          & \textbf{0.0246} \\
% 03 & \underline{0.0011} & 0.0563         & 0.0029         & 0.1019         & 0.0045         & 0.1            & \textbf{0.0009} & 0.0645         & \underline{0.0011} & \textbf{0.0321} & 0.0019         & \underline{0.0383} \\
% 04 & 0.0008         & 0.0274         & 0.0019         & 0.1356         & 0.0029         & 0.1748         & \textbf{0.0005} & 0.0348         & \underline{0.0007} & \underline{0.0256} & 0.0012         & \textbf{0.0206} \\
% 05 & 0.0012         & 0.0233         & 0.0028         & 0.0775         & 0.0033         & 0.1117         & \underline{0.0011} & 0.414          & \textbf{0.001} & \underline{0.023} & 0.0016         & \textbf{0.0218} \\
% 06 & 0.0009         & 0.0259         & 0.0023         & 0.0982         & 0.0029         & 0.112          & \textbf{0.0007} & 0.3272         & \underline{0.0008} & \underline{0.023} & 0.0013         & \textbf{0.0217} \\
% 07 & \underline{0.0013} & \textbf{0.0278} & 0.004          & 0.1149         & 0.0048         & 0.1621         & \textbf{0.0011} & 0.2353         & 0.0029         & 0.1459         & 0.0022         & \underline{0.0396} \\
% 08 & \underline{0.0013} & \underline{0.0419} & 0.0031         & 0.0822         & 0.0044         & 0.1307         & \textbf{0.0011} & 0.5395         & \textbf{0.0011} & 0.0426         & 0.0017         & \textbf{0.0404} \\
% 09 & 0.0012         & \underline{0.0245} & 0.0032         & 0.0799         & 0.0035         & 0.1369         & \textbf{0.0009} & 0.248          & \underline{0.001} & 0.0261         & 0.0016         & \textbf{0.0219} \\
% 10 & \underline{0.0015} & \textbf{0.0255} & 0.0037         & 0.0779         & 0.0043         & 0.1362         & \textbf{0.0012} & 0.1159         & 0.0018         & 0.0503         & 0.0021         & \underline{0.0328} \\
% \midrule
%  Avg. &  &  & \\
% \bottomrule
% \end{tabular}
% }
% \caption{Performance comparison of different methods on the KITTI Dataset.\\\\
%         \small{$^\star$ The estimated sequence is scale-aligned with ground truth}}
% \end{table*}


\begin{table*}[htbp]
\centering
{\fontsize{8}{9}\selectfont \textbf{Relative Position Error (RPE)}}\\
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
Traj. & 00 & 01 & 02 & 03 & 04 & 05 & 06 & 07 & 08 & 09 & 10 & Avg.\\
\midrule
\textbf{SLAM} \\
\hspace{3mm} ORB-SLAM 3         & 0.037    & \textbf{0.0419} & 0.0378   & 0.0563   & 0.0274   & 0.0233   & 0.0259   & \textbf{0.0278} & \underline{0.0419} & \underline{0.0245} & \textbf{0.0255} \\
\hspace{3mm} DROID-SLAM$^\star$ & \underline{0.0287} & 0.7194   & \underline{0.0277} & \textbf{0.0321} & \underline{0.0256} & \underline{0.023} & \underline{0.023} & 0.1459   & 0.0426   & 0.0261   & 0.0503   \\
\midrule
\textbf{VO} \\
\hspace{3mm} TartanVO$^{\star\dagger}$   & 0.385    & 3.1018   & 0.4637   & 0.268    & 1.2882   & 0.413    & 0.6619   & 0.4091   & 0.3663   & 0.5141   & 0.3281   \\
\hspace{3mm} TartanVO           & 0.1138   & 1.4809   & 0.1103   & 0.1      & 0.1748   & 0.1117   & 0.112    & 0.1621   & 0.1307   & 0.1369   & 0.1362   \\
\hspace{3mm} iSLAMVO            & 0.0877   & 0.3027   & 0.0795   & 0.1019   & 0.1356   & 0.0775   & 0.0982   & 0.1149   & 0.0822   & 0.0799   & 0.0779   \\
\hspace{3mm} DPVO$^{\star\dagger}$& 1.2781   & \underline{0.0952} & 0.634    & 0.0645   & 0.0348   & 0.414    & 0.3272   & 0.2353   & 0.5395   & 0.248    & 0.1159   \\
\midrule
\textbf{Ours}                   & \textbf{0.0284} & 0.2836   & \textbf{0.0246} & \underline{0.0383} & \textbf{0.0206} & \textbf{0.0218} & \textbf{0.0217} & \underline{0.0396} & \textbf{0.0404} & \textbf{0.0219} & \underline{0.0328} \\
\bottomrule
\multicolumn{10}{l}{\small{$^\star$ The estimated sequence is scale-aligned with ground truth.}}\\
\multicolumn{10}{l}{\small{$^\dagger$ Monocular method.}}

\end{tabular}}

{\fontsize{8}{9}\selectfont \textbf{Relative Orientation Error (ROE)}}\\
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
Traj. & 00 & 01 & 02 & 03 & 04 & 05 & 06 & 07 & 08 & 09 & 10 & Avg.\\
\midrule
\textbf{SLAM} \\
\hspace{3mm} ORB-SLAM 3         & \underline{0.0018} & \underline{0.0009} & 0.0014   & \underline{0.0011} & 0.0008   & 0.0012   & 0.0009   & \underline{0.0013} & \underline{0.0013} & 0.0012   & \underline{0.0015} \\
\hspace{3mm} DROID-SLAM$^\star$ & \textbf{0.0017} & 0.001    & \underline{0.0012} & \underline{0.0011} & \underline{0.0007} & \textbf{0.001} & \underline{0.0008} & 0.0029   & \textbf{0.0011} & \underline{0.001} & 0.0018   \\
\midrule
\textbf{VO} \\
\hspace{3mm} TartanVO$^{\star\dagger}$   & 0.0045   & 0.0038   & 0.0044   & 0.0029   & 0.0037   & 0.0034   & 0.0034   & 0.0041   & 0.0036   & 0.0047   & 0.004    \\
\hspace{3mm} TartanVO           & 0.004    & 0.0077   & 0.0035   & 0.0045   & 0.0029   & 0.0033   & 0.0029   & 0.0048   & 0.0044   & 0.0035   & 0.0043   \\
\hspace{3mm} iSLAMVO            & 0.0038   & 0.0022   & 0.0032   & 0.0029   & 0.0019   & 0.0028   & 0.0023   & 0.004    & 0.0031   & 0.0032   & 0.0037   \\
\hspace{3mm} DPVO$^{\star\dagger}$ & 0.002    & \textbf{0.0006} & \textbf{0.0011} & \textbf{0.0009} & \textbf{0.0005} & \underline{0.0011} & \textbf{0.0007} & \textbf{0.0011} & \textbf{0.0011} & \textbf{0.0009} & \textbf{0.0012} \\
\midrule
\textbf{Ours}                   & 0.0022   & 0.0043   & 0.002    & 0.0019   & 0.0012   & 0.0016   & 0.0013   & 0.0022   & 0.0017   & 0.0016   & 0.0021   \\
\bottomrule
\multicolumn{10}{l}{\small{$^\star$ The estimated sequence is scale-aligned with ground truth.}}\\
\multicolumn{10}{l}{\small{$^\dagger$ Monocular method.}}

\end{tabular}}


\caption{Performance comparison of different methods on the KITTI Dataset.}
\end{table*}


==> Sections/Table/Archive/KITTI_20240605.tex <==
% \begin{table*}[htbp]
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{cccccccccccccc}
% \toprule
%   & \multicolumn{2}{c}{{ORB-SLAM3}} & \multicolumn{2}{c}{{iSLAM-VO}} & \multicolumn{2}{c}{{TartanVO(S)}} & \multicolumn{2}{c}{{DPVO}$^\star$} & \multicolumn{2}{c}{{DROID-SLAM(S)}$^\star$} & \multicolumn{2}{c}{\textbf{Ours}} \\
% \cmidrule{2-14}
%  Traj.  &  {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} \\
% \midrule 
% 00 & \underline{0.0018} & 0.037          & 0.0038         & 0.0877         & 0.004          & 0.1138         & 0.002          & 1.2781         & \textbf{0.0017} & \underline{0.0287} & 0.0022         & \textbf{0.0284} \\
% 01 & \underline{0.0009} & \textbf{0.0419} & 0.0022         & 0.3027         & 0.0077         & 1.4809         & \textbf{0.0006} & \underline{0.0952} & 0.001          & 0.7194         & 0.0043         & 0.2836         \\
% 02 & 0.0014         & 0.0378         & 0.0032         & 0.0795         & 0.0035         & 0.1103         & \textbf{0.0011} & 0.634          & \underline{0.0012} & \underline{0.0277} & 0.002          & \textbf{0.0246} \\
% 03 & \underline{0.0011} & 0.0563         & 0.0029         & 0.1019         & 0.0045         & 0.1            & \textbf{0.0009} & 0.0645         & \underline{0.0011} & \textbf{0.0321} & 0.0019         & \underline{0.0383} \\
% 04 & 0.0008         & 0.0274         & 0.0019         & 0.1356         & 0.0029         & 0.1748         & \textbf{0.0005} & 0.0348         & \underline{0.0007} & \underline{0.0256} & 0.0012         & \textbf{0.0206} \\
% 05 & 0.0012         & 0.0233         & 0.0028         & 0.0775         & 0.0033         & 0.1117         & \underline{0.0011} & 0.414          & \textbf{0.001} & \underline{0.023} & 0.0016         & \textbf{0.0218} \\
% 06 & 0.0009         & 0.0259         & 0.0023         & 0.0982         & 0.0029         & 0.112          & \textbf{0.0007} & 0.3272         & \underline{0.0008} & \underline{0.023} & 0.0013         & \textbf{0.0217} \\
% 07 & \underline{0.0013} & \textbf{0.0278} & 0.004          & 0.1149         & 0.0048         & 0.1621         & \textbf{0.0011} & 0.2353         & 0.0029         & 0.1459         & 0.0022         & \underline{0.0396} \\
% 08 & \underline{0.0013} & \underline{0.0419} & 0.0031         & 0.0822         & 0.0044         & 0.1307         & \textbf{0.0011} & 0.5395         & \textbf{0.0011} & 0.0426         & 0.0017         & \textbf{0.0404} \\
% 09 & 0.0012         & \underline{0.0245} & 0.0032         & 0.0799         & 0.0035         & 0.1369         & \textbf{0.0009} & 0.248          & \underline{0.001} & 0.0261         & 0.0016         & \textbf{0.0219} \\
% 10 & \underline{0.0015} & \textbf{0.0255} & 0.0037         & 0.0779         & 0.0043         & 0.1362         & \textbf{0.0012} & 0.1159         & 0.0018         & 0.0503         & 0.0021         & \underline{0.0328} \\
% \midrule
%  Avg. &  &  & \\
% \bottomrule
% \end{tabular}
% }
% \caption{Performance comparison of different methods on the KITTI Dataset.\\\\
%         \small{$^\star$ The estimated sequence is scale-aligned with ground truth}}
% \end{table*}


\begin{table*}[htbp]
\centering
\captionsetup{font=small}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccccccccc}
\multicolumn{10}{l}{\textbf{Relative Translation Error ($t_{\mathrm{rel}}, \mathrm{m} / \mathrm{frame}$)}}\\
\toprule
Trajectory & 00 & 01 & 02 & 03 & 04 & 05 & 06 & 07 & 08 & 09 & 10 & Avg.\\
\midrule
\textbf{SLAM} \\
\hspace{3mm} ORB-SLAM 3         & 0.0252   & \textbf{0.0416} & 0.0438   & 0.027    & 0.0274   & 0.0161   & 0.0228   & \textbf{0.0155} & \underline{0.0271} & \underline{0.0208} & \textbf{0.0166} & \textbf{0.0258} \\
\hspace{3mm} DROID-SLAM$^\star$ & \underline{0.0198} & 0.7112   & \underline{0.0250} & \textbf{0.0182} & \underline{0.0255} & \underline{0.0153} & \underline{0.0199} & 0.0746   & 0.0275   & 0.0214   & 0.0309  & 0.0900 \\
\midrule
\textbf{VO} \\
\hspace{3mm} TartanVO$^{\star\dagger}$  & 0.2066   & 0.6834   & 0.1626   & 0.1234   & 0.1152   & 0.1821   & 0.2234   & 0.2005   & 0.1857   & 0.1704   & 0.1745  & 0.2207 \\
\hspace{3mm} TartanVO                   & 0.0656   & 1.1408   & 0.0905   & 0.0477   & 0.1747   & 0.0637   & 0.0923   & 0.0700  & 0.0721   & 0.0990   & 0.0679  & 0.1804 \\
\hspace{3mm} iSLAMVO                    & 0.0577   & 0.2978   & 0.0686   & 0.0507   & 0.1356   & 0.0504   & 0.0837   & 0.0593   & 0.0510   & 0.0660   & 0.0449  & 0.0878 \\
\hspace{3mm} DPVO$^{\star\dagger}$      & 0.4542   & \underline{0.0942} & 0.4209   & 0.0302   & 0.0348   & 0.2221   & 0.2393   & 0.1064   & 0.3051   & 0.1723   & 0.0661  & 0.1951 \\
\midrule
\textbf{Ours}                           & \textbf{0.0192} & 0.2663   & \textbf{0.0223} & \underline{0.0187} & \textbf{0.0206} & \textbf{0.0142} & \textbf{0.0187} & \underline{0.0194} & \textbf{0.0254} & \textbf{0.0182} & \underline{0.019} & \underline{0.0420} \\
\bottomrule
% \multicolumn{10}{l}{\small{$^\star$ The estimated sequence is scale-aligned with ground truth.}}\\
% \multicolumn{10}{l}{\small{$^\dagger$ Monocular method.}}
\end{tabular}}
\vspace{3mm}

\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccccccccc}
\multicolumn{10}{l}{\textbf{Relative Rotation Error ($r_{\mathrm{rel}}, \mathrm{deg} / \mathrm{frame}$)}}\\
\toprule
Trajectory & 00 & 01 & 02 & 03 & 04 & 05 & 06 & 07 & 08 & 09 & 10 & Avg.\\
\midrule
\textbf{SLAM} \\
\hspace{3mm} ORB-SLAM 3         & 0.0586   & \underline{0.0355} & 0.0529   & 0.0425   & 0.0322   & 0.0416   & 0.0338   & \underline{0.0385} & 0.0455   & 0.0444   & \underline{0.0515} & \underline{0.0434}\\
\hspace{3mm} DROID-SLAM$^\star$ & \underline{0.0538} & 0.0406   & \underline{0.0445} & \underline{0.0385} & \underline{0.0296} & \underline{0.0353} & \underline{0.0296} & 0.0734   & \underline{0.0381} & \underline{0.0378} & 0.0715  & 0.0448 \\
\midrule
\textbf{VO} \\
\hspace{3mm} TartanVO$^{\star\dagger}$   & 0.1055   & 0.0895   & 0.1105   & 0.0682   & 0.0789   & 0.0761   & 0.0816   & 0.0847   & 0.0823   & 0.1069   & 0.0907  & 0.0886 \\
\hspace{3mm} TartanVO           & 0.1026   & 0.2455   & 0.1197   & 0.0953   & 0.1158   & 0.0821   & 0.0968   & 0.0931   & 0.1063   & 0.1077   & 0.0969  & 0.1147 \\
\hspace{3mm} iSLAMVO            & 0.1052   & 0.0896   & 0.1101   & 0.0681   & 0.0787   & 0.0758   & 0.0812   & 0.0842   & 0.082    & 0.1064   & 0.0905 & 0.0883 \\
\hspace{3mm} DPVO$^{\star\dagger}$ & \textbf{0.0495} & \textbf{0.0247} & \textbf{0.0381} & \textbf{0.0330} & \textbf{0.0219} & \textbf{0.0319} & \textbf{0.0250} & \textbf{0.0311} & \textbf{0.0347} & \textbf{0.0336} & \textbf{0.0386} & \textbf{0.0329} \\
\midrule
\textbf{Ours}                   & 0.0654   & 0.1670   & 0.0715   & 0.0504   & 0.0473   & 0.0466   & 0.0456   & 0.0507   & 0.0509   & 0.0567   & 0.0569  & 0.0645 \\
\bottomrule
\multicolumn{10}{l}{\small{$^\star$ The estimated sequence is scale-aligned with ground truth.}}\\
\multicolumn{10}{l}{\small{$^\dagger$ Monocular method.}}

\end{tabular}}

\caption{Performance comparison of different methods on the KITTI Dataset.}
\end{table*}


==> Sections/Table/Archive/TartanAir_Easy_20240604.tex <==
\begin{table*}[htbp]
\centering

{\fontsize{8}{9}\selectfont \textbf{Relative Position Error (RPE)}}\\
\resizebox{\linewidth}{!}{\begin{tabular}{lccccccccccccccc}
\toprule
Traj. & E00 & E01 & E02 & E03 & E04 & E05 & E06 & E07 & E08 & E09 & E10 & E11 & E12 & E13 \\
\midrule
ORB-SLAM3           & 0.205 & - & - & - & - & 0.532 & - & - & - & - & - & - & - & -\\
DPVO$^{\star\dagger}$        & \underline{0.007} & 0.035          & \textbf{0.013} & 1.154          & 0.24           & 0.015          & \underline{0.012} & 0.027          & 0.033          & 0.302          & \underline{0.014} & 0.026          & 0.323          & 0.101          \\
DROID-SLAM$^\star$  & \textbf{0.003} & \textbf{0.02}  & 0.04           & \textbf{0.006} & \textbf{0.029} & \textbf{0.004} & \textbf{0.005} & \textbf{0.003} & \textbf{0.015} & \textbf{0.011} & \textbf{0.007} & \textbf{0.002} & \textbf{0.013} & \textbf{0.003} \\
iSLAM               & 0.136          & 0.177          & 0.204          & 0.176          & 0.157          & 0.141          & 0.126          & 0.124          & 0.139          & 0.148          & 0.184          & 0.279          & 0.493          & 0.104          \\
TartanVO$^{\star\dagger}$ & 0.426          & 0.381          & 0.924          & 0.373          & 0.884          & 0.471          & 0.466          & 0.44           & 0.641          & 0.422          & 0.399          & 0.687          & 0.85           & 1.429          \\
TartanVO         & 0.082          & 0.235          & 0.124          & 0.142          & 0.167          & 0.11           & 0.111          & 0.083          & 0.106          & 0.114          & 0.152          & 0.073          & 0.117          & 0.092          \\
\midrule
\textbf{Ours}       & 0.022          & \underline{0.028} & \underline{0.015} & \underline{0.04} & \underline{0.063} & \underline{0.012} & 0.013          & \underline{0.02} & \underline{0.026} & \underline{0.022} & 0.024          & \underline{0.01} & \underline{0.039} & \underline{0.035} \\
\bottomrule
\multicolumn{10}{l}{$^\star$ The estimated sequence is scale-aligned with ground truth}\\
\multicolumn{10}{l}{\small{$^\dagger$ Monocular method.}}
\end{tabular}}

\vspace{5mm}

{\fontsize{8}{9}\selectfont \textbf{Relative Orientation Error (ROE)}}\\
\resizebox{\linewidth}{!}{\begin{tabular}{lccccccccccccccc}
\toprule
Traj. & E00 & E01 & E02 & E03 & E04 & E05 & E06 & E07 & E08 & E09 & E10 & E11 & E12 & E13 \\
\midrule
ORB-SLAM3           & 0.148 & - & - & - & - & 0.149 & - & - & - & - & - & - & - & -\\
DPVO$^{\star\dagger}$ & \textbf{0.001} & \textbf{0.001} & \textbf{0.002} & 0.021          & \underline{0.019} & \textbf{0.001} & \textbf{0.001} & \underline{0.003} & \textbf{0.002} & 0.009          & \textbf{0.001} & \textbf{0.001} & \underline{0.005} & \underline{0.009} \\
DROID-SLAM$^\star$  & \textbf{0.001} & \textbf{0.001} & \textbf{0.002} & \textbf{0.001} & \textbf{0.004} & \textbf{0.001} & \textbf{0.001} & \textbf{0.001} & \textbf{0.002} & \textbf{0.001} & \textbf{0.001} & \textbf{0.001} & \textbf{0.003} & \textbf{0.001} \\
iSLAM               & 0.028          & 0.027          & 0.04           & 0.02           & 0.024          & 0.023          & 0.019          & 0.02           & 0.023          & 0.021          & 0.018          & 0.034          & 0.063          & 0.026          \\
TartanVO$^{\star\dagger}$ & 0.017          & 0.054          & 0.043          & 0.05           & 0.101          & 0.062          & 0.044          & 0.03           & 0.071          & 0.028          & 0.023          & 0.054          & 0.057          & 0.124          \\
TartanVO            & 0.018          & 0.014          & 0.021          & 0.026          & 0.026          & 0.018          & 0.012          & 0.027          & 0.012          & 0.012          & 0.02           & 0.017          & 0.037          & 0.024          \\
\midrule
\textbf{Ours} & \underline{0.006} & \underline{0.003} & \underline{0.004} & \underline{0.01} & 0.022          & \underline{0.003} & \underline{0.002} & 0.008          & \underline{0.005} & \underline{0.004} & \underline{0.004} & \underline{0.002} & 0.017          & 0.012          \\
\bottomrule
\multicolumn{10}{l}{$^\star$ The estimated sequence is scale-aligned with ground truth}\\
\multicolumn{10}{l}{\small{$^\dagger$ Monocular method.}}
\end{tabular}}
\caption{Performance comparison of different methods on the TartanAirV2 Test Easy. ``-'' indicates the system lost track and did not generate the estimated trajectory.}

\end{table*}


==> Sections/Table/Archive/TartanAir_Hard_20240604.tex <==

% \begin{table*}[htbp]
% \centering
% \resizebox{\linewidth}{!}{\begin{tabular}{cccccccccccccc}
% \toprule
% \multicolumn{2}{c}{\textbf{}} & \multicolumn{2}{c}{{ORB-SLAM3}} & \multicolumn{2}{c}{{iSLAM}} & \multicolumn{2}{c}{{TartanVO(S)}} & \multicolumn{2}{c}{{DPVO}} & \multicolumn{2}{c}{{DroidSLAM(S)}} & \multicolumn{2}{c}{\textbf{Ours}} \\
% \cmidrule{3-14}
%  &  & {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} \\
% \midrule
% \multirow{13}{*}{}
% & P00 &  &  &  &  & 0.024          & 0.092       & \underline{0.004}    & \textbf{0.037} & \textbf{0.001} & 0.145          & 0.011          & \underline{0.044}    \\
% & P01 &  &  &  &  & 0.037          & \underline{0.117} & 0.027          & 1.329          & \underline{0.008}    & 0.650          & \textbf{0.007} & \textbf{0.065} \\
% & P02 &  &  &  &  & 0.017          & \underline{0.073} & \textbf{0.004} & 0.077          & 0.006          & 0.206          & \underline{0.004}    & \textbf{0.024} \\
% & P03 &  &  &  &  & 0.020          & 0.152       & 0.053          & 1.127          & \textbf{0.001} & \textbf{0.015} & \underline{0.009}    & \underline{0.044}    \\
% & P04 &  &  &  &  & 0.012          & 0.114       & 0.059          & 1.308          & \textbf{0.001} & \underline{0.111}    & \underline{0.011}    & \textbf{0.094} \\
% & P05 &  &  &  &  & 0.012          & 0.106       & 0.016          & 0.518          & \textbf{0.001} & \textbf{0.002} & \underline{0.002}    & \underline{0.010}    \\
% & P06 &  &  &  &  & 0.027          & 0.083       & \underline{0.002}    & 0.058          & \textbf{0.001} & \textbf{0.009} & 0.006          & \underline{0.043}    \\
% & P07 &  &  &  &  & 0.012          & \underline{0.111} & 0.027          & 0.790          & \textbf{0.003} & 0.144          & \underline{0.004}    & \textbf{0.017} \\
% & P08 &  &  &  &  & 0.018          & 0.110       & 0.012          & 0.156          & \textbf{0.003} & \underline{0.062}    & \underline{0.005}    & \textbf{0.042} \\
% & P09 &  &  &  &  & 0.026          & 0.167       & 0.144          & 2.622          & \textbf{0.001} & \textbf{0.009} & \underline{0.015}    & \underline{0.065}    \\
% & P10 &  &  &  &  & 0.026          & 0.142       & 0.016          & 0.563          & \textbf{0.001} & \textbf{0.003} & \underline{0.011}    & \underline{0.034}    \\
% & P11 &  &  &  &  & 0.021          & 0.124       & 0.006          & 0.192          & \textbf{0.002} & \underline{0.091}    & \underline{0.004}    & \textbf{0.019} \\
% & P12 &  &  &  &  & \textbf{0.014} & 0.235       & 0.065          & 0.898          & \underline{0.025}    & \underline{0.233}    & 0.037          & \textbf{0.086} \\
% & P13 &  &  &  &  & \underline{0.018}    & \underline{0.082} & 0.233          & 3.632          & \textbf{0.005} & \textbf{0.078} & 0.029          & 0.082          \\
%  \midrule
% & Avg &  &  &  &  & 0.020          & \underline{0.122} & 0.048          & 0.951          & \textbf{0.004} & 0.126          & \underline{0.011}    & \textbf{0.048} \\
% \bottomrule
% \end{tabular}}
% \caption{Performance comparison of different methods on the TartanAirV2 Test.}
% \end{table*}



\begin{table*}[htbp]
\centering

{\fontsize{8}{9}\selectfont \textbf{Relative Position Error (RPE)}}\\
\resizebox{\linewidth}{!}{\begin{tabular}{lccccccccccccccc}
\toprule
Traj. & H00 & H01 & H02 & H03 & H04 & H05 & H06 & H07 & H08 & H09 & H10 & H11 & H12 & H13 & Avg. \\
\midrule
\textbf{SLAM} \\
\hspace{3mm}DROID-SLAM$^\star$   & \textbf{0.037} & \underline{0.135} & 0.107          & \textbf{0.008} & \textbf{0.031} & \textbf{0.003} & \textbf{0.009} & \underline{0.025} & \textbf{0.028} & \textbf{0.011} & \textbf{0.005} & \underline{0.023} & 0.851          & \underline{0.101} & \underline{0.126} \\
\midrule
\textbf{VO} \\
\hspace{3mm}iSLAM-VO                  & 0.152          & 0.223          & 0.093          & 0.114          & 0.281          & 0.202          & 0.277          & 0.272          & 0.174          & 0.164          & 0.155          & 0.154          & \underline{0.193} & 0.256          & 0.699 \\
\hspace{3mm}TartanVO$^{\star\dagger}$ & 0.844          & 0.639          & 1.016          & 0.668          & 0.701          & 0.977          & 0.825          & 1.631          & 0.597          & 3.66           & 0.683          & 0.838          & 0.699          & 1.557          & 1.095 \\
\hspace{3mm}TartanVO                  & 0.195          & 0.434          & 0.189          & 0.239          & 0.403          & 0.217          & 0.263          & 0.189          & 0.18           & 0.198          & 0.213          & 0.199          & 0.209          & 0.199          & 0.238 \\
\hspace{3mm}DPVO$^{\star\dagger}$     & \textbf{0.037} & 1.329          & \underline{0.077} & 1.127          & 1.308          & 0.518          & 0.058          & 0.79           & 0.156          & 2.622          & 0.563          & 0.192          & 0.898          & 3.632         & 0.951 \\
\midrule
\textbf{Ours} & \underline{0.044} & \textbf{0.065} & \textbf{0.024} & \underline{0.044} & \underline{0.094} & \underline{0.01} & \underline{0.043} & \textbf{0.017} & \underline{0.042} & \underline{0.065} & \underline{0.034} & \textbf{0.019} & \textbf{0.086} & \textbf{0.082} & \textbf{0.048}\\
\bottomrule
\multicolumn{10}{l}{\small{$^\star$ The estimated sequence is scale-aligned with ground truth.}}\\
\multicolumn{10}{l}{\small{$^\dagger$ Monocular method.}}
\end{tabular}}

\vspace{5mm}

{\fontsize{8}{9}\selectfont \textbf{Relative Orientation Error (ROE)}}\\
\resizebox{\linewidth}{!}{\begin{tabular}{lccccccccccccccc}
\toprule
Traj. & H00 & H01 & H02 & H03 & H04 & H05 & H06 & H07 & H08 & H09 & H10 & H11 & H12 & H13 & Avg. \\
\midrule
\textbf{SLAM} \\
\hspace{3mm}DROID-SLAM$^\star$ & \textbf{0.001} & \underline{0.008} & \underline{0.006} & \textbf{0.001} & \textbf{0.001} & \textbf{0.001} & \textbf{0.001} & \textbf{0.003} & \textbf{0.003} & \textbf{0.001} & \textbf{0.001} & \textbf{0.002} & \underline{0.025} & \textbf{0.005} & \textbf{0.004}\\
\midrule
\textbf{VO} \\
\hspace{3mm}iSLAM-VO & 0.027          & 0.031          & 0.021          & 0.045          & 0.029          & 0.051          & 0.065          & 0.055          & 0.039          & 0.03           & 0.065          & 0.025          & \textbf{0.024} & 0.041          & 0.162\\
\hspace{3mm}TartanVO$^{\star\dagger}$ & 0.078          & 0.341          & 0.177          & 0.204          & 0.201          & 0.222          & 0.218          & 0.274          & 0.146          & 0.454          & 0.156          & 0.191          & 0.256          & 0.368          & 0.235\\
\hspace{3mm}TartanVO & 0.059          & 0.03           & 0.026          & 0.04           & 0.045          & 0.044          & 0.026          & 0.048          & 0.021          & 0.024          & 0.051          & 0.048          & 0.07           & 0.059          & 0.042\\
\hspace{3mm}DPVO$^{\star\dagger}$ & \underline{0.004} & 0.027          & \textbf{0.004} & 0.053          & 0.059          & 0.016          & \underline{0.002} & 0.027          & 0.012          & 0.144          & 0.016          & 0.006          & 0.065          & 0.233          & 0.048\\
\midrule
\textbf{Ours} & 0.011          & \textbf{0.007} & \textbf{0.004} & \underline{0.009} & \underline{0.011} & \underline{0.002} & 0.006          & \underline{0.004} & \underline{0.005} & \underline{0.015} & \underline{0.011} & \underline{0.004} & 0.037          & \underline{0.029} & \underline{0.011}\\
\bottomrule
\multicolumn{10}{l}{\small{$^\star$ The estimated sequence is scale-aligned with ground truth.}}\\
\multicolumn{10}{l}{\small{$^\dagger$ Monocular method.}}
\end{tabular}}
\caption{Performance comparison of different methods on the TartanAirV2 Test Hard. Additional results on ``Easy'' trajectories of TartanAir v2 are in \aref{appendix:AdditionalResults}. Noticably, ORB-SLAM3 lost track on all hard sequences and is therefore not included in this table. \\\\
        \small{$^\star$ The estimated sequence is scale-aligned with ground truth}}
\end{table*}


==> Sections/Table/Archive/TartanAir_Hard_20240605.tex <==

% \begin{table*}[htbp]
% \centering
% \resizebox{\linewidth}{!}{\begin{tabular}{cccccccccccccc}
% \toprule
% \multicolumn{2}{c}{\textbf{}} & \multicolumn{2}{c}{{ORB-SLAM3}} & \multicolumn{2}{c}{{iSLAM}} & \multicolumn{2}{c}{{TartanVO(S)}} & \multicolumn{2}{c}{{DPVO}} & \multicolumn{2}{c}{{DroidSLAM(S)}} & \multicolumn{2}{c}{\textbf{Ours}} \\
% \cmidrule{3-14}
%  &  & {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} & {{r\_rel}} & {{t\_rel}} \\
% \midrule
% \multirow{13}{*}{}
% & P00 &  &  &  &  & 0.024          & 0.092       & \underline{0.004}    & \textbf{0.037} & \textbf{0.001} & 0.145          & 0.011          & \underline{0.044}    \\
% & P01 &  &  &  &  & 0.037          & \underline{0.117} & 0.027          & 1.329          & \underline{0.008}    & 0.650          & \textbf{0.007} & \textbf{0.065} \\
% & P02 &  &  &  &  & 0.017          & \underline{0.073} & \textbf{0.004} & 0.077          & 0.006          & 0.206          & \underline{0.004}    & \textbf{0.024} \\
% & P03 &  &  &  &  & 0.020          & 0.152       & 0.053          & 1.127          & \textbf{0.001} & \textbf{0.015} & \underline{0.009}    & \underline{0.044}    \\
% & P04 &  &  &  &  & 0.012          & 0.114       & 0.059          & 1.308          & \textbf{0.001} & \underline{0.111}    & \underline{0.011}    & \textbf{0.094} \\
% & P05 &  &  &  &  & 0.012          & 0.106       & 0.016          & 0.518          & \textbf{0.001} & \textbf{0.002} & \underline{0.002}    & \underline{0.010}    \\
% & P06 &  &  &  &  & 0.027          & 0.083       & \underline{0.002}    & 0.058          & \textbf{0.001} & \textbf{0.009} & 0.006          & \underline{0.043}    \\
% & P07 &  &  &  &  & 0.012          & \underline{0.111} & 0.027          & 0.790          & \textbf{0.003} & 0.144          & \underline{0.004}    & \textbf{0.017} \\
% & P08 &  &  &  &  & 0.018          & 0.110       & 0.012          & 0.156          & \textbf{0.003} & \underline{0.062}    & \underline{0.005}    & \textbf{0.042} \\
% & P09 &  &  &  &  & 0.026          & 0.167       & 0.144          & 2.622          & \textbf{0.001} & \textbf{0.009} & \underline{0.015}    & \underline{0.065}    \\
% & P10 &  &  &  &  & 0.026          & 0.142       & 0.016          & 0.563          & \textbf{0.001} & \textbf{0.003} & \underline{0.011}    & \underline{0.034}    \\
% & P11 &  &  &  &  & 0.021          & 0.124       & 0.006          & 0.192          & \textbf{0.002} & \underline{0.091}    & \underline{0.004}    & \textbf{0.019} \\
% & P12 &  &  &  &  & \textbf{0.014} & 0.235       & 0.065          & 0.898          & \underline{0.025}    & \underline{0.233}    & 0.037          & \textbf{0.086} \\
% & P13 &  &  &  &  & \underline{0.018}    & \underline{0.082} & 0.233          & 3.632          & \textbf{0.005} & \textbf{0.078} & 0.029          & 0.082          \\
%  \midrule
% & Avg &  &  &  &  & 0.020          & \underline{0.122} & 0.048          & 0.951          & \textbf{0.004} & 0.126          & \underline{0.011}    & \textbf{0.048} \\
% \bottomrule
% \end{tabular}}
% \caption{Performance comparison of different methods on the TartanAirV2 Test.}
% \end{table*}



\begin{table*}[htbp]
\centering
\captionsetup{font=small}
\resizebox{\linewidth}{!}{\begin{tabular}{lccccccccccccccc}
\multicolumn{10}{l}{\textbf{Relative Translation Error ($t_{\mathrm{rel}}, \mathrm{m} / \mathrm{frame}$)}}\\
\toprule
Trajectory & H00 & H01 & H02 & H03 & H04 & H05 & H06 & H07 & H08 & H09 & H10 & H11 & H12 & H13 & Avg. \\
\midrule
\textbf{SLAM} \\
\hspace{3mm}DROID-SLAM$^\star$        & \textbf{0.009} & \underline{0.048} & 0.029          & \textbf{0.005} & \textbf{0.014} & \textbf{0.002} & \textbf{0.006} & \underline{0.008} & \underline{0.019} & \textbf{0.006} & \textbf{0.004} & \underline{0.006} & 0.146          & \underline{0.031} & \underline{0.024} \\
\midrule
\textbf{VO} \\
\hspace{3mm}iSLAM-VO                  & 0.182          & 0.423          & 0.341          & 0.370          & 0.422          & 0.307          & 0.382          & 0.215          & 0.325          & 0.362          & 0.259          & 0.258          & 0.257          & 0.210         & 0.308 \\
\hspace{3mm}TartanVO$^{\star\dagger}$ & 0.097          & 0.160          & 0.315          & 0.194          & 0.247          & 0.292          & 0.234          & 0.261          & 0.272          & 0.277          & 0.245          & 0.220          & 0.164          & 0.235         & 0.230 \\
\hspace{3mm}TartanVO                  & 0.067          & 0.150          & 0.070          & 0.098          & 0.150          & 0.091          & 0.106          & 0.073          & 0.072          & 0.084          & 0.082          & 0.068          & \underline{0.080} & 0.078       & 0.091 \\
\hspace{3mm}DPVO$^{\star\dagger}$     & \underline{0.010} & 0.498          & \underline{0.025} & 0.290          & 0.308          & 0.174          & 0.024          & 0.240          & 0.054          & 0.385          & 0.164          & 0.048          & 0.189          & 0.336    & 0.196 \\
\midrule
\textbf{Ours} & 0.011          & \textbf{0.028} & \textbf{0.008} & \underline{0.017} & \underline{0.033} & \underline{0.005} & \underline{0.017} & \textbf{0.006} & \textbf{0.016} & \underline{0.024} & \underline{0.011} & \textbf{0.005} & \textbf{0.027} & \textbf{0.027} & \textbf{0.017}\\
\bottomrule
% \multicolumn{10}{l}{\small{$^\star$ The estimated sequence is scale-aligned with ground truth.}}\\
% \multicolumn{10}{l}{\small{$^\dagger$ Monocular method.}}
\end{tabular}}


\vspace{3mm}

\resizebox{\linewidth}{!}{\begin{tabular}{lccccccccccccccc}
\multicolumn{10}{l}{\textbf{Relative Rotation Error ($r_{\mathrm{rel}}, {}^\circ / \mathrm{frame}$)}}\\
\toprule
Trajectory & H00 & H01 & H02 & H03 & H04 & H05 & H06 & H07 & H08 & H09 & H10 & H11 & H12 & H13 & Avg. \\
\midrule
\textbf{SLAM} \\
\hspace{3mm}DROID-SLAM$^\star$ & \textbf{0.033} & \underline{0.117} & 0.080          & \textbf{0.032} & \textbf{0.026} & \textbf{0.021} & \textbf{0.025} & \textbf{0.053} & \textbf{0.082} & \textbf{0.030}  & \textbf{0.060}  & \textbf{0.026} & \textbf{0.236} & \textbf{0.091} & \textbf{0.065}\\
\midrule
\textbf{VO} \\
\hspace{3mm}iSLAM-VO & 3.337          & 2.630          & 2.557          & 3.085          & 2.776          & 3.018          & 2.423          & 3.307          & 2.189          & 2.435          & 2.874          & 2.899          & 3.755          & 3.145         & 2.888 \\
\hspace{3mm}TartanVO$^{\star\dagger}$ & 0.459          & 3.338          & 2.629          & 2.556          & 3.084          & 2.775          & 3.017          & 2.423          & 3.305          & 2.191          & 2.435          & 2.874          & 2.899          & 3.756         & 2.696 \\
\hspace{3mm}TartanVO & 0.751          & 0.433          & 0.382          & 0.637          & 0.724          & 0.754          & 0.398          & 0.794          & 0.327          & 0.405          & 0.809          & 0.657          & 1.186          & 0.946         & 0.657 \\
\hspace{3mm}DPVO$^{\star\dagger}$ & \underline{0.077} & 0.494          & \underline{0.079} & 2.418          & 0.654          & 0.711          & \underline{0.066} & 0.682          & 0.254          & 2.703          & 0.250          & 0.187          & 1.430          & 2.943         & 0.925 \\
\midrule
\textbf{Ours} & 0.120          & \textbf{0.115} & \textbf{0.058} & \underline{0.140} & \underline{0.168} & \underline{0.044} & 0.090          & \underline{0.066} & \underline{0.085} & \underline{0.252} & \underline{0.162} & \underline{0.053} & \underline{0.604} & \underline{0.484} & \underline{0.174}\\
\bottomrule
\multicolumn{10}{l}{\small{$^\star$ The estimated sequence is scale-aligned with ground truth.}}\\
\multicolumn{10}{l}{\small{$^\dagger$ Monocular method.}}
\end{tabular}}
\caption{Performance comparison of different methods on the TartanAir v2 Test Hard. Additional results on \textit{Easy} trajectories of TartanAir v2 are in \aref{appendix:AdditionalTartanAirv2}. Noticably, ORB-SLAM3 lost track on all hard sequences and is therefore not included in this table.}
\end{table*}


==> Sections/Table/TartanAir2_Hard_even.tex <==
\begin{table*}[ht]
\centering
\captionsetup{font=small}
\caption{Relative motion error on the TartanAir v2 Hard Dataset. Only even numbered trajectories in the Hard subset are shown here. For odd-numbered trajectories in the Hard subset, see \tref{tab: TartanAirHard Odd}. ORB-SLAM3 lost track of all trajectories and is therefore not shown in the table.}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccccccccccc}
\toprule
 Trajectory & \multicolumn{2}{c}{{H00}} & \multicolumn{2}{c}{{H02}} & \multicolumn{2}{c}{{H04}} & \multicolumn{2}{c}{H06} & \multicolumn{2}{c}{H08} & \multicolumn{2}{c}{H10} & \multicolumn{2}{c}{H12}\\
% \cmidrule{2-15}
   &  $t_{\mathrm{rel}}$ & $r_{\mathrm{rel}}$ & $t_{\mathrm{rel}}$ & $r_{\mathrm{rel}}$ & $t_{\mathrm{rel}}$ & $r_{\mathrm{rel}}$ & $t_{\mathrm{rel}}$ & $r_{\mathrm{rel}}$ & $t_{\mathrm{rel}}$ & $r_{\mathrm{rel}}$ & $t_{\mathrm{rel}}$ & $r_{\mathrm{rel}}$ & $t_{\mathrm{rel}}$ & $r_{\mathrm{rel}}$\\
\midrule
\textbf{SLAM} \\
\hspace{3mm} DROID-SLAM$^\star$         & \textbf{0.009} & \textbf{0.033} & 0.029          & 0.080 & \textbf{0.014} & \textbf{0.026} & \textbf{0.006} & \textbf{0.025} & \underline{0.019} & \textbf{0.082} & \textbf{0.004} & \textbf{0.060} & 0.146 & \textbf{0.236}\\
\midrule
\textbf{VO} \\
\hspace{3mm} iSLAM-VO                    & 0.182          & 3.337 & 0.341          & 2.557 & 0.422          & 2.776 & 0.382          & 2.423 & 0.325          & 2.189 & 0.259          & 2.874 & 0.257          & 3.755 \\
\hspace{3mm} TartanVO$^{\star\dagger}$  & 0.097          & 0.459 & 0.315          & 2.629 & 0.247          & 3.084 & 0.234          & 3.017 & 0.272          & 3.305 & 0.245          & 2.435 & 0.164          & 2.899 \\
\hspace{3mm} TartanVO                   & 0.067          & 0.751 & 0.070          & 0.382 & 0.150          & 0.724 & 0.106          & 0.398 & 0.072          & 0.327 & 0.082          & 0.809 & \underline{0.080} & 1.186 \\
\hspace{3mm} DPVO$^{\star\dagger}$      & \underline{0.010} & \underline{0.077} & \underline{0.025} & \underline{0.079} & 0.308          & 0.654 & 0.024          & \underline{0.066} & 0.054          & 0.254 & 0.164          & 0.250 & 0.189          & 1.430 \\
\midrule 
\textbf{Ours}                           & 0.011          & 0.120 & \textbf{0.008} & \textbf{0.058} & \underline{0.033} & \underline{0.168} & \underline{0.017} & 0.090 & \textbf{0.016} & \underline{0.085} & \underline{0.011} & \underline{0.162} & \textbf{0.027} & \underline{0.604} \\
\bottomrule
\multicolumn{10}{l}{\small{$^\star$ The estimated sequence is scale-aligned with ground truth.}}\\
\multicolumn{10}{l}{\small{$^\dagger$ Monocular method.}}\\
\end{tabular}
}
\vspace{-10pt}
\label{tab: TartanAirHard Even}
\end{table*}


